Modeling Spatiotemporal Periodicity and Collaborative Signal for Local-Life Service Recommendation

Online local-life service platforms provide services like nearby daily essentials and food delivery for hundreds of millions of users. Different from other types of recommender systems, local-life service recommendation has the following characteristics: (1) spatiotemporal periodicity, which means a user's preferences for items vary from different locations at different times. (2) spatiotemporal collaborative signal, which indicates similar users have similar preferences at specific locations and times. However, most existing methods either focus on merely the spatiotemporal contexts in sequences, or model the user-item interactions without spatiotemporal contexts in graphs. To address this issue, we design a new method named SPCS in this paper. Specifically, we propose a novel spatiotemporal graph transformer (SGT) layer, which explicitly encodes relative spatiotemporal contexts, and aggregates the information from multi-hop neighbors to unify spatiotemporal periodicity and collaborative signal. With extensive experiments on both public and industrial datasets, this paper validates the state-of-the-art performance of SPCS.

==> 03ref/010introduction.tex <==


% intro草稿 by chx
% 主要围绕：图拓扑结构的演化性 + 节点特征的演化性 --> 分开建模
% 1. 动态图协同过滤的优势
% 2. 两个主要问题：（1）动态图更加稀疏；（2）动态图联合建模拓扑和特征的演化性导致低度节点学习的不好
% 3. 现有的SSL方法的局限性 -- 提出问题
% 4. 我们的方法

Recommender systems have been widely deployed to discover users' preferences in numerous online services, such as e-commerce, online reviews and videos \cite{zhou2018deep,an2019neural}. 
% 早期推荐的方法使用XXX技术讲user/item“单独”映射到embedding空间。这些方法通过隐式反馈挖掘user/item之间的潜在关系，而
Earlier collaborative filtering methods \cite{rendle2012bpr,he2017neural} projects single ID of each user/item into embedding. 
In order to exploit high-order connection in user-item static graph, graph collaborative filtering methods \cite{wang2019neural,he2020lightgcn} apply graph neural networks to learn effective node representations. Since the users' preferences evolve over time, some works \cite{kang2018selfattentive,sun2019bert4rec,li2020time} leverage historical time-ordered item sequence to predict future items for users, called sequential methods. 
However, the performance of both graph collaborative filtering and sequential methods is far from satisfactory: the former do not take temporal evolution into account, while the latter do not take high-order collaborative filtering into account. 
To overcome such limitations, temporal graph collaborative filtering (TGCF) models the interaction data on user-item temporal graph and apply temporal graph neural networks \cite{kumar2019predicting,trivedi2019dyrep,xu2020inductive,rossi2020temporal} to capture the evolution of topology and feature, which are widely used in continuous-time sequential recommendation. 

% As an effective approach, graph collaborative filtering (GCF) \cite{wang2019neural,he2020lightgcn} organizes historical interactions as a user-item static graph to integrate high-order information into node representations for recommendation. Recently, GCF is further enhanced by the powerful temporal graph neural networks (TGNN) \cite{kumar2019predicting,trivedi2019dyrep,xu2020inductive,rossi2020temporal}, which introduce timestamps to capture the evolution of user-item temporal graph and then applies TGNN to learn node representations for recommendation, called \textit{temporal graph collaborative filtering} (TGCF). 

Despite the remarkable success, existing TGCF methods still suffer from data sparsity issue \cite{sarwar2001sparsity,wu2021self}. The user-item static graph, which is usually sparse, can be regarded as the last snapshot after time accumulation, while the user-item temporal graph at each timestamp can be regarded as a subset of the static graph.
Therefore, the user-item temporal graph are more vulnerable to data sparsity issue than user-item static graph. For instance, the average degrees of a static graph from 2000-04-05 to 2014-07-02 on Garden are 10.02, while that of temporal graph at 2009-07-27 are 2.12. As a result, the graph-based collaborative methods that heavily rely on the graph topology are easily biased to the node degrees \cite{chen2020bias,tang2020investigating}, resulting in the unfairness between the nodes with high degree and low degree, leading to the representations of long-tail nodes unreliable. As shown in Figure \ref{fig:long-tail-ndcg}, we can observe that the lower the degree is, the larger the numbers and the lower the NDCG@20 of nodes have. More concretely, if a user/item has fewer historical interactions, it is hard to directly learn its representation and evolution. 

Despite the remarkable success, existing TGCF methods still suffer from an open problem, \textbf{skewed data distribution} \cite{sarwar2001sparsity,wu2021self} based on graph models.   The static graph of interactions can be regarded as the last snapshot after time accumulation, and usually exhibits a power-law distribution, where the long tail consisting of low-degree items can rarely dominate the training/learning of GCNs.  Due to the sparse data of temporal graphs, which is a series of snapshots split by timestamp to capture the temporal evolution, the problem of skewed data distribution is more serious.
While the temporal graph is a series of snapshots split by timestamp to capture the temporal evolution. skewed data distribution is more important in TGN. Existing TGCF methods adopt the message-passing scheme to model the evolution of topology and feature in a unified framework, which are easily biased towards high-degree nodes \cite{chen2020bias,tang2020investigating} on a such sparse user-item temporal graph, leading to the representations of long-tail nodes unreliable. In contrast, high-degree items appear more frequently in neighborhood aggregation, thus exerting a more significant impact on representation learning. Hence, the TGCFs are easily biased toward high-degree items, sacrificing the performance of low-degree (long-tail) items, which means modeling the evolution of topology and ignoring feature learning.

\begin{figure}
\centering
% \quad
\subfigure[Degree distribution.]{
\includegraphics[width=0.475\linewidth]{02fig/powerlow-garden.pdf}
}
% \quad
\subfigure[NDCG@20 of TGCF backbones.]{
\includegraphics[width=0.475\linewidth]{02fig/intro-ndcg-garden.pdf}
}
\caption{Long-tail recommendation on Garden.}
\label{fig:long-tail-ndcg}
\end{figure}

Existing studies attempt to alleviate the sparsity of interaction data from two aspects: graph topology and node feature. Earlier works adopt generative methods, such as Variational AutoEncoder (VAE), to learn the local posterior distribution of node feature, which decreases the vulnerability to the long-tail issue. However, these methods ignore high-order collaborative filtering, which prevent VAE from achieving satisfactory performance. To tackle this limitation, another line of research adopt graph augmentation and contrastive learning into graph collaborative filtering backbones (e.g. LigthGCN). They first augmenting the user-item static graph and then calculate the contrastive loss for multi-task training, which distills additional signal for long-tail nodes. However, since these methods still model the topology and feature in a unified framework to learn the whole distribution of the graph rather than a single node, the long-tail issue of topology always has a negative effective on the distribution learning of node feature. In other word, high-degree nodes appear more frequently in neighborhood aggregation, thus expert larger impact on representation learning (especially for long-tail nodes). Besides, most of existing works are applied to static graph-based recommender systems and ignore the evolution of graph topology and feature, which is essential for temporal graph-based recommender systems. 

% Existing studies attempt to alleviate the sparsity of interaction data from two aspects: graph topology and node feature. One line of research augments the user-item static graph with structure perturbations and then adopt contrastive learning to maximize the agreement between different views. These methods focus more on graph topology, which distill additional signal for long-tail nodes. Another line of research mainly focus on the distribution of node features. They adopt generative methods, such as Variational AutoEncoder (VAE), to learn the posterior distribution or add random uniform noises to the original features to enhance model robustness, which decreases the vulnerability to the sparse issue. However, few of studies consider both topology and feature for long-tail nodes, in which the framework is hard to design and less scalable. Besides, these methods are applied to static graph-based recommender systems and ignore the evolution of graph topology and feature, which is essential for temporal graph-based recommender systems.

% Self-supervised learning (SSL) has been studied in CV \cite{gidaris2018unsupervised,oord2018representation} and NLP \cite{devlin2018bert,lan2019albert} to distill additional signal through the unlabeled data space, which achieves remarkable improvements in downstream tasks. To alleviate the sparsity of interaction data, existing studies \cite{wu2021self,yu2022graph,lin2022improving,zhou2021selfcf} leverage self-supervised learning in recommendation, which can be categorized into two branches: generative methods and contrastive methods. Early works adopt generative methods, such as Variational AutoEncoder (VAE), to learn the local posterior distribution, which decreases the vulnerability to the sparse issue. However, these methods ignore high-order collaborative filtering, which prevent VAE from achieving satisfactory performance. Another line of contrastive methods first augmenting the user-item static graph and then adopt contrastive learning to maximize the agreement between different views. However, these methods focus on the whole distribution of the graph rather than a single node (like a VAE) neglect local distribution of the neighborhood. Besides, both of generative and contrastive methods ignore the evolution of graph topology and feature, which is essential for temporal graph-based recommender systems. In summary, how to capture the evolution of graph topology and feature under serious data sparsity issue in temporal graph remains unclear. 

% Although several recent studies \cite{wu2021self,yu2022graph,lin2022improving,zhou2021selfcf} leverage self-supervised learning (SSL) in recommendation to alleviate the sparsity of interaction data, they are limited to solve aforementioned issues: 1) these methods mainly aim to enhance user-item static graph, ignoring the temporal evolution of topology and feature; 2) they focus on global augmentation concerning the properties of the whole distribution of the graph rather than a single node and neglect local distribution of the neighborhood; 3) since they modify the graph adjacent matrix, they are not scalable enough especially in user-item temporal graph. In view of these issues and limitations, a follow-up question then arises: \textit{Are there effective and scalable approaches that address the data sparsity issue on temporal graph-based recommender systems?}

In this work, in order to learn effective node representations (especially for low-degree nodes), we propose a novel framework: \textbf{T}emporal \textbf{L}ocal \textbf{A}ugmentation for Temporal Graph Collaborative Filtering (\modelname-TGCF), which models the distribution and evolution of topology and feature separately. To be specific, for topology distribution and evolution modeling, we utilize memory mechanism, which stores one-hop temporal structure information and is updated based on timestamps. 
For feature distribution and evolution modeling, we utilize \modelname to enhance the node representations. First, we split several snapshots based on timestamps. For each snapshot, we propose a pretraining step to learn the conditional distribution of the connected neighbors' node features given one center node's feature via a generative model \cite{kingma2013auto,sohn2015learning}. Then, we exploit this distribution to generate \modelname node features based on memory, and fuse them with time series function \cite{medsker2001recurrent,graves2012long,chung2014empirical} to capture the evolution of node representations. Furthermore, we decouple the pretraining step and downstream TGCF training, allowing our \modelname is model-agnostic and to be applied to not only TGCF methods but also other recommender methods, such as general \cite{he2020lightgcn} and sequential methods \cite{kang2018selfattentive,li2020time,fan2021continuoustime}. Last but not least, we fuse memory and generated augmentation node features as input for TGCF methods. 

We verify the effective of our \modelname-TGCF framework on five real-world datasets. Extensive experiment results for recommendation show that our \modelname achieves new state-of-the-art performance. Besides, our proposed \modelname outperforms other SSL methods, such as SGL \cite{wu2021self}, SimGCL \cite{yu2022graph} and NCL \cite{lin2022improving}, which demonstrates the superiority of our method. Our contributions can be summarized threefold:
\begin{itemize}[leftmargin=*]
    \item We first propose the influence of data sparsity issue on user-item temporal graph for recommendation, and analyze the inaccuracy of modeling the evolution of topology and feature in a unified framework for low-degree nodes, which provides a future direction.
    \item We propose \modelname-TGCF framework, which utilize memory and \modelname to capture the distribution and evolution of topology and feature separately. Particularly, \modelname is model-agnostic and scalable, which can be applied to various popular backbones. 
    \item Extensive experiments on five public datasets demonstrate that our method can alleviate data sparsity issue on temporal graph-based recommender systems. 
\end{itemize}



==> 04other/000abstract.tex <==



Online local-life service platforms provide services like nearby daily essentials and food delivery for hundreds of millions of users. 
Different from conventional e-commerce platforms, 
% the users’ preferences for items vary from different regions at different times due to the geographical limitations and living habits.
(1) the users' locations change periodically, and they constantly tend to order items close to their locations;
(2) the users' preferences for items change periodically with respect to their locations as well as regular living habits.
In this work, we summarize it as the \textbf{region-aware periodic} problem, which was not well-studied in previous studies.
Although existing recommender systems have tackled the problem of modeling transitions from spatial or temporal contexts, their performance in solving the region-aware periodic problem for local-life service recommendation is limited. 
% they cannot effectively solve the region-aware periodic problem for local-life service recommendation.
To address this issue, we propose a novel method named \modelname in this paper.
First, to capture the spatial-temporal contexts for periodic modeling, we design the \textit{periodic encoding} with both temporal and geographical encoding.
% in \modelname. 
Second, we design the \textit{geographical temporal graph transformer} with periodic encoding to capture the region-aware periodic.
%First, it  \textit{periodic encoding} is proposed with temporal encoding and geographical encoding to capture the spatial-temporal contexts for periodic modeling.
%Then, the \textit{geographical temporal graph transformer} with periodic encoding is further proposed to capture the region-aware periodic.
With extensive experiments on both public and industrial datasets, this paper validates the state-of-the-art performance of \modelname.




==> 04other/012introduction.tex <==


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\linewidth]{02fig/local-periodic.png}
%     \vspace{-0.1in}
%     \caption{The distribution of visited POIs of user-1767 on \industry dataset. Different colors represent POIs visited by the user in different time periods: blue denotes 10:00-16:00, and red denotes 18:00-24:00. The radius of the circle is 700m.}
%     \label{fig:intro-spatial}
%     \vspace{-0.2in}
% \end{figure}

\begin{figure}[t]
% \vspace{-0.1in}
\centering
% \subfigure[Two days.]{ % 2-21 $\sim$ 2-22
% \includegraphics[width=0.475\linewidth]{02fig/time-periodic-day-2.pdf}
% }
\subfigure[The motivation example.]{ % 2-21 $\sim$ 2-22
\includegraphics[width=0.455\linewidth]{02fig/local-periodic-5.png}
}
% \quad
\subfigure[Location changes over two days.]{ % 3-17 $\sim$ 3-18
\includegraphics[width=0.495\linewidth]{02fig/time-local-periodic-2.pdf}
}
% \subfigure[Interaction periodic over two weeks.]{
% \includegraphics[width=0.97\linewidth]{02fig/time-periodic-week-2.pdf}
% }
\vspace{-0.2in}
\caption{Illustration of region-aware periodic on \industry dataset. (a) is an example for user-1767 where different colors represent his/her interacted items in different regions at different times: blue denotes the time period of 10:00-14:00, whereas red is 18:00-22:00 (circle radius is 500m). (b) is the statistic of the average distance between each user’s consecutive locations (of interactions) over two days.}
\label{fig:intro-spatial}
\vspace{-0.2in}
\end{figure}


Online local-life service platforms, such as Meituan\footnote{\url{http://i.meituan.com/}} and Uber Eats\footnote{\url{https://www.ubereats.com/}}, provide services like nearby daily essentials and food delivery for hundreds of millions of users.
Different from conventional e-commerce platforms \cite{zhou2018deep,zhou2019deep}, users' preferences for items vary from different regions at different times due to geographical limitations and living habits, as illustrated by an example in Figure \ref{fig:intro-spatial}(a).
% , a user tends to order takeaways near the office at noon whereas to visit restaurants near home in the evening.
Compared with other types of recommender systems, local-life service recommendation faces the following challenges:
% (2) \textit{region periodic}.
(1) The users' locations change periodically, and they tend to interact with items geographically close to their locations. %  limitations.
% Through observation and statistics illustrated in Figure \ref{fig:intro-spatial}(b), when 
For instance, a user will travel from home to the workplace in the morning and return home in the evening.
% According to our statistics in Figure \ref{fig:intro-spatial}(b), 
Through the statistics in Figure \ref{fig:intro-spatial}(b), we notice that there is a large distance between users' consecutive locations in the morning and evening, indicating the change of location is highly relevant to the time.
% (1) \textit{preference periodic}. 
(2) Under the impact of locations and regular living habits, users change their preferences for items periodically. % due to the combined influence of their locations and regular living habits. 
They tend to interact with (via clicking or purchasing) similar items from different regions at specific times, such as buying coffee near the workplace every morning but ordering fast food near home at night.
% buy KFC burgers every Thursday night.
% , and some users may like to order Starbucks coffee every morning.
All these characteristics have important implications for local-life service recommendation yet have rarely been studied in existing works. 
We summarize the challenges as a \textbf{region-aware periodic} problem.
In this paper, we focus on modeling such region-aware periodic in local-life service platforms.


% Point-of-Interest (POI) recommendation has plenty of applications in industrial scenarios \cite{islam2022survey,sanchez2022point}.
% Distinct from traditional POI scenarios, \textit{local-life services}, which have achieved great success recently, incorporate location-based information to suggest nearby life services for users at a specific time. 
% For instance, Meituan\footnote{\url{http://www.meituan.com}} recommends an enormous variety of local-life services to users, including food delivery, shop recommendations, etc. From the perceptive of users, the local-life services offer a more personal browsing experience. 
% Users could access local services anytime and anywhere.
% The local-life services have brought both opportunities and challenges to POI recommendation, especially the \textit{spatial-temporal periodic} involved. 
% In general, the spatial-temporal periodic mainly reflects that the user prefers POIs in different regions at different times due to geographical restrictions. 
% In a specific example, as Figure \ref{fig:intro-spatial} shows, a user tends to order takeaways near the company at noon whereas to visit restaurants near home in the evening.



% The spatial-temporal periodic is mainly observed in two aspects: %points:
% \textit{interaction periodic} and \textit{region periodic}. \textbf{First}, the \textit{interaction periodic} is that user-POI interactions exhibit periodic of multiple granularities, which means the interaction occurs or recurs at regular time intervals. 
% As shown in Figure \ref{fig:intro-spatial}(c), we find that during the week, users have more interactions on weekends than on weekdays; as shown in Figure \ref{fig:intro-spatial}(a), during the day, noon and evening are peak times for all users visiting restaurants. 
% \textbf{Second}, the \textit{region periodic} is that users' geographic changes exhibit periodic.
% For instance, users will travel from home to office in the morning and return home in the evening.
% According to our statistics in Figure \ref{fig:intro-spatial}(b), we notice that users' location changes dramatically in the morning and evening, which indicates that such a region periodic is significantly related to time. 

Generally speaking, there are two relevant lines of research for local-life service recommendation.
One is the next POI (Point-of-Interest) Recommendation. 
The majority of studies about POI recommenders \cite{liu2016predicting,sun2020go,luo2021stan,ma2018point,lian2020geography} directly utilize time intervals or spatial distance between current and future steps to capture the transitional regularities, without taking the periodicity of user preferences into consideration. 
A few works \cite{feng2018deepmove,sun2020go,cui2021st} model the user preferences from long-term behaviors for multi-level periodicity \cite{feng2018deepmove}, but they do not explicitly encode the region-aware periodic.
% These methods capture the dynamics of user preference, are not time-aware and cannot explicitly encode the periodicity. 
Another line of research is periodic-related recommenders. 
Recent periodic-related works \cite{wang2019modeling,fan2021continuoustime,rossi2020temporal,tian2022temporal} aim to encode the periodicity by utilizing time interval contexts and time-decaying functions.
% But these methods are time-sensitive, they mainly focus on the most recent interactions to model the user's current intentions (i.e. short-term intentions).
However, these methods fail to utilize the spatial-temporal contexts to capture the region-aware periodic, where users' preferences are strongly influenced by their locations.
In short, the above existing solutions leave a blank space in addressing the region-aware periodic problem for local-life service recommendation.

% However, existing works lack the ability to capture such spatial-temporal periodic.
% Most existing POI methods \cite{liu2016predicting,sun2020go,luo2021stan} simply utilize time intervals between current and future steps to capture the evolution, ignoring the interaction periodic. 
% A few works \cite{feng2018deepmove,sun2020go,cui2021st} aim to model long-term user preferences from historical check-ins for multi-level periodic \cite{feng2018deepmove}, but do not explicitly encode the interaction periodic.
% To capture the interaction periodic, some recent works \cite{fan2021continuoustime,zhang2022dynamic} apply temporal graph neural networks \cite{trivedi2019dyrep,xu2020inductive,rossi2020temporal} for continuous-time recommendation, but fail to utilize the geographical context for region periodic.
% Besides, simply capturing the spatial distance between two consecutive steps without considering the interaction periodic as previous works \cite{ma2018point,lian2020geography}, can hardly reflect the region periodic. 

To address this issue, we propose \modelname, a novel \textbf{R}egion-\textbf{A}ware \textbf{P}eriodic \textbf{G}raph Network for local-life service recommendation.
First, to capture the spatial-temporal contexts for periodic modeling, we design the \textit{periodic encoding}, which explicitly encodes the time interval as \textit{temporal encoding} and the spatial distance as \textit{geographical encoding}.
Second, to further capture the region-aware periodic, we design a novel \textit{geographical temporal graph transformer}, which combines temporal encoding and geographical encoding.
The main contributions of this paper are as follows:
\begin{itemize}[leftmargin=*]
    \item To the best of our knowledge, we take the first step to investigate the region-aware periodic problem for local-life service recommendation.
    \item We propose a novel \modelname method to solve the region-aware periodic problem. 
    Specifically, we capture the spatial-temporal contexts as the periodic encoding, and then design the geographical temporal graph transformer with periodic encoding to further capture the region-aware periodic.
    \item We conduct extensive experiments on both real-world public and industrial datasets. Experimental results demonstrate the effectiveness of our proposed \modelname.
\end{itemize}





==> 04other/020definition.tex <==




% In this section, we give problem formulations and term definitions. 
% Let $\mathcal{U}$ be a set of users, $\mathcal{P}$ be a set of POIs, $\mathcal{C}$ be a set of locations with latitude and longitude coordinates, and $\mathcal{T}$ be the time set. 

\begin{mydef}
    \textbf{Spatial-Temporal User-POI Graph} is defined as $\mathcal{G} = \{\mathcal{U}, \mathcal{P}, \mathcal{E}\}$, where $\mathcal{U}$ represents a set of users, $\mathcal{P}$ is a set of POIs, $\mathcal{E}$ is a set of temporal edges. Each edge $e_{u, p}^{t} \in \mathcal{E}$ is denoted as a quintuple, $e_{u, p}^{t} = (u, p, t, g_{u}^t, g_p)$, where $u \in \mathcal{U}$, $p \in \mathcal{P}$, $t \in \mathbb{R}^+$, $\{g_{u}^t, g_p\} \subset \mathcal{C}$, and $\mathcal{C}$ is a set of locations notated as tuples of their latitude and longitude. Each $(u, p, t, g_{u}^t, g_p)$ means that a user $u$ at location $g_{u}^t$ and time $t$ visits the POI $p$ that locates in $g_p$.
    We denote $\mathcal{N}_{u}^t = \{(p, t_p, g_p) \ | \ e_{u, p}^{t_p} \in \mathcal{E}, t_p < t\}$ as the temporal neighborhood set of user $u$ in time interval $[0, t)$. 
    % The temporal neighbor $p$ for user $u$ at time $t$ can be defined as $\mathcal{N}_{u}^t = \{(p, t_p) \ | \ e_{u, p}^{t_p} \in \mathcal{E}, t_p < t\}$. 
\end{mydef}

\begin{mydef}
    \textbf{Local-Life Service Recommendation.} Given a spatial-temporal user-POI graph $\mathcal{G}$ and a new query tuple $(u, t, g_{u}^t)$, it aims to recommend POIs that user $u$ would be interested at time $t$ and location $g_u^t$. 
\end{mydef}

% \begin{definition}(Continuous-Time Sequential Recommendation)
%     Continuous-time sequential recommendation task \cite{fan2021continuoustime} is defined as:
%     \begin{itemize}[leftmargin=*]
%         \item \textbf{Given:} A user set $\mathcal{U}$, an item set $\mathcal{I}$, and a CTTG $\mathcal{G}$.
%         \item \textbf{Question:} Calculate the final temporal embeddings $\mathbf{H}_{\mathcal{U}}(t)$ for users and $\mathbf{H}_{\mathcal{I}}(t)$ for items to estimate probabilities that a user in the CTTG will interact with items, and then return ranking lists of items at a set of future timestamps $\mathcal{T}_u$.
%     \end{itemize}
% \end{definition}

==> 04other/030method.tex <==


In this section, we first present related terms and formalize the problem of local-life service recommendation, then introduce the three main parts of our \modelname: 
(1) \textit{periodic encoding}, which explicitly encodes the time interval as temporal encoding and the spatial distance as geographical encoding.  
(2) \textit{geographical temporal graph transformer}, which combines these encodings to capture the region-aware periodic. 
(3) the prediction and optimization. 
Figure \ref{fig:method-framework} illustrates the overall structure of \modelname. 


\subsection{Problem Formulation}

\begin{mydef}
    \textbf{Spatial-Temporal User-Item Graph} is defined as $\mathcal{G} = \{\mathcal{U}, \mathcal{I}, \mathcal{E}\}$, where $\mathcal{U}$ and $\mathcal{I}$ is the set of users and items, $\mathcal{E}$ is a set of temporal edges. Each edge $e_{u, i}^{t} \in \mathcal{E}$ is denoted as a quintuple, $e_{u, i}^{t} = (u, i, t, p_{u}^t, p_i)$, where $u \in \mathcal{U}$, $i \in \mathcal{I}$, $t \in \mathbb{R}^+$, $\{p_{u}^t, p_i\} \subset \mathcal{P}$, and $\mathcal{P}$ is a set of locations with latitude and longitude. Each $(u, i, t, p_{u}^t, p_i)$ means that a user $u$ will interact with item $i$ at time $t$, traveling from location $p_{u}^t$ to location $p_{i}$, where $p_{u}^t$ is the latest visited location of user $u$ before time $t$.
    We denote $\mathcal{N}_{u}^t = \{(i, t_i, p_i) \ | \ e_{u, i}^{t_i} \in \mathcal{E}, t_i < t\}$ as the temporal neighborhood set of user $u$ in time interval $[0, t)$. 
    % The temporal neighbor $p$ for user $u$ at time $t$ can be defined as $\mathcal{N}_{u}^t = \{(p, t_p) \ | \ e_{u, p}^{t_p} \in \mathcal{E}, t_p < t\}$. 
\end{mydef}

\begin{mydef}
    \textbf{Local-Life Service Recommendation.} Given a spatial-temporal user-item graph $\mathcal{G}$ and a new query tuple $(u, t, p_{u}^t)$, local-life service recommendation aims to recommend item list that user $u$ would be interested at time $t$ and location $p_u^t$. 
\end{mydef}

\subsection{Periodic Encoding}\label{sec:periodic-encoding}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{02fig/GeoTGN-v6.pdf}
    \vspace{-0.2in}
    \caption{The overall framework of our proposed \modelname.}
    \label{fig:method-framework}
    \vspace{-0.1in}
\end{figure}

\subsubsection{\textbf{Memory State and Hidden Embedding}}

To maintain each user’s (item’s) history in a compressed format, we adopt a widely-used memory mechanism \cite{rossi2020temporal}. 
First, the memory state for a user $u$ (item $i$) at time $t$ is denoted as $\bm{s}_{u}^t$ ($\bm{s}_{i}^t$) $\in \mathbb{R}^c$, initialized as an all-zero vector and updated by the memory mechanism. 
Then, we define $\bm{h}_u^{(\ell - 1), t}$ as the hidden embedding that serves as the input to the $\ell$-th layer for user $u$ at time $t$ (the same applies to the hidden embedding for item $i$).
Note that, in the first layer, $\bm{h}_u^{(0), t} = s_u^t$. %\textit{i.e.} the memory state.
When $\ell > 1$, it is generated from the previous layer.

% For instance, to update $\bm{s}_u^t$ for user $u$ at time $t$, we first sample its temporal neighbors $(p, t_p)\in \mathcal{N}_{u}^t$, and then the proceeds --- \textit{Message Function}, \textit{Message Aggregator}, and \textit{Memory Updater} --- can be formulated as: 
% \begin{gather}
%     \mathbf{m}_{u \leftarrow p}^{t_p} = [\bm{s}_u^{t^-} \| \bm{s}_p^{t_p} \| \phi(t - t_p)] \\
%     \mathbf{\overline{m}}_{u}^t = \mathrm{Agg}\left\{\mathbf{m}_{u \leftarrow p}^{t_p} \ | \ (p, t_p) \in \mathcal{N}_{u}^t \right\} \\
%     \bm{s}_u^t = \mathrm{Mem}(\overline{\mathbf{m}}_u^t, \bm{s}_u^{t^-})
% \end{gather}
% where $[ \cdot \| \cdot]$ denotes vector concatenate, $\mathbf{s}_{u}^{t{-}}$ is the latest state of user $u$ before time $t$.
% $\mathrm{Agg}\{\cdot\}$ denotes aggregation function, such as mean and last time aggregation \cite{rossi2020temporal}.  
% $\mathrm{Mem}(\cdot)$ represents a time series function and we use GRU \cite{chung2014empirical} in this paper.



\subsubsection{\textbf{Temporal Encoding (TE)}}

Inspired by recent works \cite{xu2020inductive, fan2021continuoustime}, the periodicity can be reflected by the time intervals between the user's different interactions. 
We use a generic time encoding function as $\phi(\cdot) \rightarrow \mathbb{R}^{c_t}$ based on Bochner’s Theorem \cite{loomis2013introduction} to encode the time intervals into embedding explicitly.
Specifically, given two time points $t_1$ and $t_2$, and the time interval is defined as $\Delta t = |t_2 - t_1|$, we implement $\phi(\cdot)$ as:
% To capture the periodic of multiple granularities, we adopt a generic time encoding function \cite{xu2020inductive} based on Bochner’s Theorem \cite{loomis2013introduction} to obtain the continuous-time embedding $\phi(\cdot) \in \mathbb{R}^{c_t}$ for specific time intervals. 
% Specifically, given two time points $t_1$ and $t_2$, $\Delta t = |t_2 - t_1|$, we implement $\phi(\cdot)$ as: 
\begin{equation}
    \phi(\Delta t) = \left[\cos(\omega_1 \Delta t + b_1), \cdots, \cos(\omega_{c_t} \Delta t + b_{c_t})\right],
\end{equation}
where $\bm{\omega} = [\omega_1, \cdots, \omega_{c_t}]$ and $\bm{b} = [b_1, \cdots, b_{c_t}]$ are learnable weights and bias of linear transformation for time interval $\Delta t$. 

\subsubsection{\textbf{Geographical Encoding (GE)}}
To quantify the change of locations between different users and items, we adopt the spatial distance function called \textit{Haversine formula} \cite{robusto1957cosine} to derive the geographical scalar $d(\cdot, \cdot)$. 
Specifically, given two locations represented by their respective latitude and longitude, $p_1 = (x_1, z_1)$ and $p_2 = (x_2, z_2)$, the $d(p_1, p_2)$ is calculated as: 
\begin{equation}
    d(p_1, p_2) = \mathrm{Haversine}(x_1, z_1, x_2, z_2),
\end{equation}
where the unit of $d(p_1, p_2)$ is kilometer (km).



\subsubsection{\textbf{Region-Aware Periodic Modeling}}

To capture the region-aware periodic, we aim to incorporate temporal encoding, geographical encoding, and hidden embeddings as follows.
First, given a query user $(u, t, p_u^t)$ and its temporal neighbor $(i, t_i, p_i) \in \mathcal{N}_u^t$, we concatenate the hidden embedding and temporal encoding as $\bm{h}_i^{(\ell-1), t_i} \, \| \, \phi(t - t_i)$. 
Second, to further capture the region-aware periodic, we combine the embedding generated in the first step and geographical encoding into $\frac{\bm{h}_i^{(\ell-1), t_i} \, \| \, \phi(t - t_{i})}{[d(p_{u}^t, p_{i}) / \tau] + 1}$.
The intuition is that region-aware periodic is highly relevant to both time and nearby items, and this combination allows capturing both aspects.
% Finally, we can combine all these encodings to capture both the interaction periodic and region periodic. 
% $\frac{\bm{h}^{(\ell-1), t_p}_p  \,\|\, \phi(t - t_{p})}{d(g_{u}^t, g_{p}) + 1}$


\subsection{Geographical Temporal Graph Transformer}

To capture the region-aware periodic, we propose the geographical temporal graph transformer, which explicitly encodes the periodicity with temporal encoding and geographical encoding.
It has two operations: 
(1) construction of query, key, and value; (2) temporal self-attention.
In the following, we take the calculation for user $u$ at time $t$ as an example.
% , while the operation of item $i$ is analogous.

% In this section, we describe the geographical temporal graph transformer in two steps: (i) construction of query, key, and value; (ii) temporal self-attention mechanism to aggregate information from temporal neighbors.
% In the following, we take the calculation for user $u$ at time $t$ as an example, while the process is analogous to POI $p$. 

\subsubsection{\textbf{Construction of Query, Key and Value}}

As mentioned in Section \ref{sec:periodic-encoding}, given the query user $(u, t, p_u^t)$, we construct the query vector $\bm{q}^{(\ell), t}$ for user $u$ itself at $\ell$-th layer as:
\begin{equation}\label{equ:query}
    \bm{q}^{(\ell), t} = \frac{\bm{h}_u^{(\ell-1), t} \, \| \, \phi(t - t)}{[d(p_{u}^t, p_{u}^{t}) / \tau] + 1} = \bm{h}_u^{(\ell-1), t} \, \| \, \phi(0), 
\end{equation}
where the layer number $\ell = \{1, \cdots,L\}$. $\tau$ is used to control the decay rate of the weights and we set $\tau = 1$ in this paper. 
% $d(\cdot, \cdot)$ denotes the distance metric and we adopt \textit{Haversine formula} \cite{robusto1957cosine} in this paper. 
% Note that when $\ell = 1$, the hidden embedding $\bm{h}_u^{(\ell-1), t} = \bm{h}_u^{(0), t} = s_u^t$, \textit{i.e.} the memory state. 
% When $\ell > 1$, it is generated from the previous layer.
% Since $\phi(\cdot)$ can capture temporal periodic as mentioned in \cite{xu2020inductive}, we further consider the distance between different users and POIs. 
% The motivation is that, in a local-life service platform like Meituan, users will prioritize nearby POIs in a short period of time rather than faraway POIs. 
In addition to query user $u$ itself, we also construct key and value from user $u$'s temporal neighbors $(i, t_i, p_i)\in \mathcal{N}_{u}^t$. 
Similar to the construction of the query vector, the key/value matrix for all user $u$'s temporal neighbors can be formulated as: 
\begin{equation}\label{equ:key-value}
    \mathbf{K}^{(\ell), t} = \mathbf{V}^{(\ell), t} = \begin{bmatrix}
    % \frac{\bm{h}^{(\ell-1), t_1}_1  \,\|\, \phi(t - t_{1})}{d(g_{u}^t, g_{1}) + 1}\\
    \cdots \\
     \frac{\bm{h}^{(\ell-1), t_i}_i  \,\|\, \phi(t - t_{i})}{[d(p_{u}^t, p_{i}) / \tau] + 1} \\
    %  [1.5ex]
    \cdots
    \end{bmatrix}.
\end{equation}

\subsubsection{\textbf{Temporal Self-Attention}}

% To obtain the hidden user/POI embeddings, we adopt a self-attention mechanism \cite{vaswani2017attention} with the residual connection that leverages query, key, and value as follows: 
Then, we adopt a self-attention mechanism to obtain the hidden user (item) embeddings and utilize the residual connection to prevent over-smoothing \cite{li2020deepergcn} as follows:
\begin{equation}\label{equ:attn}
    % \tilde{\bm{h}}_u^{(\ell), t} = (\mathbf{W}_v^{(\ell)} \mathbf{V}^{(\ell), t}) \cdot \mathrm{Softmax}\left(\frac{(\mathbf{W}_k^{(\ell)} \mathbf{K}^{(\ell), t})^{\top} (\mathbf{W}_q^{(\ell)} \bm{q}^{(\ell), t})}{\sqrt{d + d_{t}}}\right) 
    \tilde{\bm{h}}_u^{(\ell), t} = \left(\mathbf{W}_v^{(\ell)} \mathbf{V}^{(\ell), t}\right) \cdot \sigma\left(\frac{[\mathbf{W}_k^{(\ell)} \mathbf{K}^{(\ell), t}]^{\top} [\mathbf{W}_q^{(\ell)} \bm{q}^{(\ell), t}]}{\sqrt{c + c_{t}}}\right),
\end{equation}
\begin{equation}\label{equ:residual}
    \bm{h}_u^{(\ell), t} = \mathrm{MLP}(\bm{h}_u^{(\ell-1), t} \, \|\, \tilde{\bm{h}}_u^{(\ell), t}),
\end{equation}
where $\sigma(\cdot)$ is the softmax function in this part. $\mathbf{W}_{q}^{(\ell)}, \mathbf{W}_{k}^{(\ell)}, \mathbf{W}_{v}^{(\ell)}  \in \mathbb{R}^{c\times (c+c_t)}$ are learnable transformation matrices at $\ell$-th layer. 
% Then, we adopt residual connection to alleviate over-smoothing: 
% \begin{equation}\label{equ:residual}
%     \bm{h}_u^{(\ell), t} = \mathrm{MLP}\left(\bm{h}_u^{(\ell-1), t} \, \|\, \tilde{\bm{h}}_u^{(\ell), t}\right).
% \end{equation}
In the last layer $L$, we can obtain the final embedding for user $u$ as $\bm{h}_{u}^t = \bm{h}_{u}^{(L),t}$. Analogously, for item $i$, we need to alternate the user information to item information, and change the neighbor information in Eq. (\ref{equ:query}), (\ref{equ:key-value}) and (\ref{equ:attn}) according to user-item pairs. Thus, $\bm{h}_{i}^t$ for item $i$ can also be calculated. 


\subsection{Prediction and Optimization}

For each $(u, i, t, p_u^t, p_i)$, we can calculate the affinity score $y_{u, i}^t = \mathrm{MLP} (\bm{h}_{u}^t \| \bm{h}_{i}^t)$ between user $u$ and item $i$ at time $t$.
% \begin{equation}
%     y_{u, p}^t = \mathrm{MLP} (\bm{h}_{u}^t \| \bm{h}_{p}^t).
% \end{equation}
To optimize parameters, we utilize the widely-used pairwise BPR loss \cite{rendle2012bpr} for top-K recommendation, which can be formulated as:
\begin{equation}
    \mathcal{L} = \sum_{u \in \mathcal{U}} \sum_{(u, i, i', t) \in \mathcal{O}} -\ln \sigma \left(y_{u, i}^t - y_{u, i'}^t\right) + \lambda \| \bm{\theta} \|_2^2,
\end{equation}
where $\mathcal{O} = \{(u, i, i', t) \ | \ e_{u, i}^t \in \mathcal{E} , e_{u, i'}^{t} \notin \mathcal{E}\}$ denotes the pairwise training data, and $\sigma(\cdot)$ is the sigmoid function. $ \lambda \| \bm{\theta} \|_2^2$ denotes the $L_2$ regularization for addressing over-fitting. 

==> 04other/040experiment.tex <==




\subsection{Experimental Settings}

\begin{table}[t]
\caption{Statistics of Datasets.}
\vspace{-0.1in}
\label{tab:datasets}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccc}
\hline
% \toprule
\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{\#Users}} & \multicolumn{1}{c}{\textbf{\#Items}} & \multicolumn{1}{c}{\textbf{\#Instances}} & \textbf{Timespan}           \\ 
\hline
% \midrule
Gowalla-Food                         & 15,058                               & 26,594                                & 553,121                                  & 2009-01-21 $\sim$ 2010-03-11 \\
\industry                              & 17,862                               & 26,236                                & 649,101                                  & 2022-02-14 $\sim$ 2022-03-28 \\ 
\hline
% \bottomrule
\end{tabular}
}
\vspace{-0.1in}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[htp]
\caption{Comparison results on two datasets. \ul{Underline} means the best baseline, and \textbf{bold} means the best performance. We report the average and standard deviation over 3 independent runs.}
\vspace{-0.1in}
\label{tab:all}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}c|cccc|cccc@{}}
% \toprule
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{4}{c|}{\textbf{Gowalla-Food}}                                                                                                                                            & \multicolumn{4}{c}{\textbf{\industry}}                                                                                                                                                 \\ 
% \cmidrule(l){2-5}  \cmidrule(l){6-9}
\cline{2-5} \cline{6-9}
\multicolumn{1}{c|}{}                                & \multicolumn{1}{c}{\textbf{Hit@10}}     & \multicolumn{1}{c}{\textbf{Hit@20}}     & \multicolumn{1}{c}{\textbf{NDCG@10}}       & \textbf{NDCG@20}                            & \multicolumn{1}{c}{\textbf{Hit@10}}     & \multicolumn{1}{c}{\textbf{Hit@20}}     & \multicolumn{1}{c}{\textbf{NDCG@10}}       & \textbf{NDCG@20}                           \\ 
% \midrule
\hline
LightGCN                                             & \multicolumn{1}{c}{0.0337±0.0001}          & \multicolumn{1}{c}{0.0562±0.0003}          & \multicolumn{1}{c}{0.0109±0.0001}          & 0.0142±0.0001                               & \multicolumn{1}{c}{0.0380±0.0002}          & \multicolumn{1}{c}{0.0646±0.0002}          & \multicolumn{1}{c}{0.0179±0.0001}          & 0.0205±0.0001                              \\
ST-RNN                                                & \multicolumn{1}{c}{0.0264±0.0002}          & \multicolumn{1}{c}{0.0397±0.0001}          & \multicolumn{1}{c}{0.0189±0.0001}          & 0.0222±0.0001                               & \multicolumn{1}{c}{0.0185±0.0002}          & \multicolumn{1}{c}{0.0357±0.0003}          & \multicolumn{1}{c}{0.0098±0.0001}          & 0.0131±0.0001                              \\
SAE-NAD                                              & \multicolumn{1}{c}{0.0873±0.0043}          & \multicolumn{1}{c}{0.1314±0.0049}          & \multicolumn{1}{c}{0.0541±0.0019}          & 0.0678±0.0020                               & \multicolumn{1}{c}{0.0555±0.0013}          & \multicolumn{1}{c}{0.0938±0.0022}          & \multicolumn{1}{c}{0.0379±0.0008}          & 0.0512±0.0012                              \\
% DyRep                                                & \multicolumn{1}{c}{0.0901±0.0085}          & \multicolumn{1}{c}{0.1263±0.0115}          & \multicolumn{1}{c}{0.0536±0.0056}          & 0.0627±0.0063                               & \multicolumn{1}{c}{0.0435±0.0026}          & \multicolumn{1}{c}{0.0752±0.0019}          & \multicolumn{1}{c}{0.0213±0.0019}          & 0.0292±0.0017                              \\
% TGN                                                  & \multicolumn{1}{c|}{\ul{0.2440}±0.0046}    & \multicolumn{1}{c|}{{\ul{0.3041}±0.0029}}    & \multicolumn{1}{c|}{{\ul{0.1692}±0.0064}}    & {\ul{0.1843}±0.0059}                         & \multicolumn{1}{c|}{{\ul{0.0902}±0.0037}}    & \multicolumn{1}{c|}{{\ul{0.1448}±0.0076}}    & \multicolumn{1}{c|}{{\ul{0.0604}±0.0033}}    & {\ul{0.0769}±0.0044}                        \\ 
\hline
% \midrule
TGSRec & 0.1595±0.0163  & 0.2141±0.0116 & 0.1071±0.0205 & 0.1208±0.0194 & 0.0619±0.0007 & 0.0998±0.0010 & 0.0315±0.0006 & 0.0409±0.0006 \\
SLRC-BPR & 0.1837±0.0014 & 0.2262±0.0008 & 0.1390±0.0012 & 0.1441±0.0015 & 0.1053±0.0010 & 0.1650±0.0016 & 0.0516±0.0011 & 0.0580±0.0011 \\
TGN-attn                                                  & \multicolumn{1}{c}{{0.2440}±0.0046}    & \multicolumn{1}{c}{{{0.3041}±0.0029}}    & \multicolumn{1}{c}{{{0.1692}±0.0064}}    & {{0.1843}±0.0059}                         & \multicolumn{1}{c}{{{0.0902}±0.0037}}    & \multicolumn{1}{c}{{{0.1448}±0.0076}}    & 0.0468±0.0024 & 0.0604±0.0033                        \\ 
TGN-R5km                                                 & \multicolumn{1}{c}{\ul{0.3047}±0.0009}    & \multicolumn{1}{c}{{\ul{0.3847}±0.0012}}    & \multicolumn{1}{c}{{\ul{0.1891}±0.0003}}    & {\ul{0.2145}±0.0004}                         & \multicolumn{1}{c}{{\ul{0.1425}±0.0055}}    & \multicolumn{1}{c}{{\ul{0.2160}±0.0092}}    & \multicolumn{1}{c}{{\ul{0.0767}±0.0035}}    & {\ul{0.0951}±0.0044}                        \\ 
% \midrule
\hline
\textbf{\modelname}                                      & \multicolumn{1}{c}{\textbf{0.3576}±0.0007} & \multicolumn{1}{c}{\textbf{0.3931}±0.0014} & \multicolumn{1}{c}{\textbf{0.2931}±0.0010} & \multicolumn{1}{c|}{\textbf{0.3021}±0.0008} & \multicolumn{1}{c}{\textbf{0.1863}±0.0013} & \multicolumn{1}{c}{\textbf{0.2662}±0.0026} & \multicolumn{1}{c}{\textbf{0.1073}±0.0007} & \textbf{0.1273}±0.0008 \\ 
% \bottomrule
\hline
\end{tabular}
}
\vspace{-0.1in}
\end{table*}

\subsubsection{Dataset} 
We conduct experiments on two real-world datasets: Gowalla-Food
% \footnote{\url{http://www.yongliu.org/datasets.html}} 
\cite{liu2014exploiting} and \industry. 
Gowalla-Food is a location-based service network for recommendation research.
The \industry dataset is collected from one of the largest local-life service platforms in China. 
Each interaction contains a user-ID, item-ID, timestamp, and GPS locations. 
For each dataset, we use the 10-core settings in \cite{he2020lightgcn} and chronologically split for train, validation, test in 8:1:1. 
The statistics of all datasets are summarized in Table \ref{tab:datasets}.




\subsubsection{Baselines} 
We compare our \modelname with several baselines. 
LightGCN \cite{he2020lightgcn} is a widely-used method for graph collaborative filtering. 
ST-RNN \cite{liu2016predicting} and SAE-NAD \cite{ma2018point} leverage spatial and temporal contexts for the next POI recommendation. 
TGSRec \cite{fan2021continuoustime}, SLRC \cite{wang2019modeling}, and TGN \cite{rossi2020temporal} are periodic-related recommenders. 
For SLRC, we choose its BPR version as SLRC-BPR.
For TGN, we choose its attention version as TGN-attn, and then further enhance it as TGN-R5km by limiting the recall within a 5km radius.

\subsubsection{Implementation and Evaluation} 
We implement our \modelname with PyTorch \cite{paszke2019pytorch} and conduct experiments on NVIDIA A100 GPU (80GB). 
We apply the Adam optimizer and the default node dimension $c$ and time dimension $c_t$ are set to 128. 
We tune the learning rate in \{1e-3, 1e-4, 1e-5\}, and search $\tau$ from \{1, 2, 5\}.
For interaction in the test set, we perform a full ranking \cite{he2020lightgcn} with all item candidates to evaluate the top-K recommendation performance, including Hit@K and NDCG@K, where K in \{10, 20\}.







\subsection{Overall Performance}

Table \ref{tab:all} shows the performance comparison between our \modelname and baselines. 
The observations from the table are: 
(1) \modelname consistently outperforms all the baselines on two datasets. 
In particular, \modelname improves over the strongest baseline \textit{w.r.t} Hit@10 by 17.36\% and 30.73\% on Gowalla-Food and \industry datasets, respectively. 
The superiority of our \modelname lies in explicitly modeling the region-aware periodic with periodic encoding and geographical temporal graph transformer. 
(2) Periodic-related recommenders (TGSRec, SLRC-BPR, TGN-attn, and TGN-R5km) generally perform better than POI (ST-RNN and SAE-NAD) and other recommenders. 
This validates the importance of explicitly encoding the periodicity for local-life service recommendation.
% (3) TGN, which only captures the interaction periodic without region periodic, outperforms two spatial-temporal methods (ST-RNN and SAE-NAD) for POI recommendation.
% This indicates the importance of modeling interaction periodic in local-life service recommender systems.
(3) Recalling within 5km improves the performance of TGN-attn, but the performance of TGN-R5km is still worse than our \modelname. 
The reason is that our \modelname explicitly captures the region-aware periodic in the training stage, whereas TGN-R5km only utilizes spatial contexts in the inference stage. 
(4) ST-RNN performs even worse than LightGCN in most cases, indicating the lack of high-order collaborative signals. 


\begin{figure}[t]
\vspace{-0.05in}
\centering
\subfigure[Prediction results of user-1767.]{
\includegraphics[width=0.49\linewidth]{02fig/heatmap_1767-2.pdf}
}
% \quad
\subfigure[Predicted location changes.]{
\includegraphics[width=0.46\linewidth]{02fig/pred-time-local-periodic-2.pdf}
}
\vspace{-0.2in}
\caption{Periodic analysis of \modelname on \industry dataset. (a) denotes the prediction results of user-1767 over a period of time. (b) denotes the average distance between each user’s consecutive locations (of predictions) over two days.}
\label{fig:contribution-2}
\vspace{-0.1in}
\end{figure}

\begin{figure}[tp]
\centering
% \vspace{-0.1in}
\subfigure[TGN-R5km.]{
\includegraphics[width=0.4\linewidth]{02fig/local_5-result-2.png}
}
% \quad
\subfigure[\modelname.]{
\includegraphics[width=0.4\linewidth]{02fig/geotgn-final-result.png}
}
\vspace{-0.2in}
\caption{Case study for user-994 over a period of time on \industry dataset. The black mark denotes the user's latest visited location, green marks denote the user's target items at different times, blue marks denote the top-5 predicted items, and red marks denote the hit items. The inner blue circle and outer green circle denote a 2km and 5km radius.}
\label{fig:contribution}
\vspace{-0.1in}
\end{figure}

\subsection{Model Analysis of \modelname}

\subsubsection{Periodic Analysis}
To explore the region-aware periodic modeling of \modelname, we first choose the same user as in Figure \ref{fig:intro-spatial}(a) and predict its preference for items over a period of time.
As shown in Figure \ref{fig:contribution-2}(a), the prediction reflects that the user prefers different items at different times.
Moreover, we further made statistics of the average distance between each user’s consecutive locations (of predictions) over time.
As shown in Figure \ref{fig:contribution-2}(b), we find that the distribution of the predicted location changes is similar to the one depicted in Figure \ref{fig:intro-spatial}(b).
% In conclusion, the aforementioned analysis further demonstrates the effectiveness of our \modelname.


\subsubsection{Case Study}
 
To further investigate the effectiveness of our \modelname, we conduct a case study comparing \modelname with TGN-R5km on \industry dataset. 
% As shown in Table xxxx, we observe that simple recall within 5km improves the performance of TGN. 
% However, it is still worse than our \modelname.
% This might be that our \modelname not only learns the geographical information, but also captures the spatial-temporal periodic patterns. 
% Besides, case study in Figure \ref{fig:contribution} further demonstrates the observation. 
As shown in Figure \ref{fig:contribution}, the user's target items are mostly located within 2km, and \modelname performs better than TGN-R5km in hitting these items.
This further demonstrates the importance of capturing the region-aware periodic for local-life service recommendation. 

\subsubsection{Ablation Study}

We further conduct an ablation study to validate two encodings in \modelname.
As shown in Table \ref{tab:ablation}, variants (1) and (2) refer to \modelname without using the temporal encoding (TE) or geographical encoding (GE), respectively.
We can observe that both variants (1) and (2) suffer from severe performance degradation on two datasets. 
This indicates that both spatial-temporal contexts are crucial for region-aware periodic modeling.
Besides, variant (2) has more performance degradation than variant (1), indicating that the spatial context is more important than the temporal context for local-life service recommendation.



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\caption{Ablation study for \modelname on two datasets.}
\vspace{-0.1in}
\label{tab:ablation}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l|cc|cc@{}}
% \toprule
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{2}{c|}{\textbf{Gowalla-Food}} & \multicolumn{2}{c}{\textbf{\industry}}  \\ 
% \cmidrule(l){2-3} \cmidrule(l){4-5} 
\cline{2-5} 
\multicolumn{1}{c|}{}                                & \multicolumn{1}{c}{\textbf{Hit@10}}   & \textbf{NDCG@10}   & \textbf{Hit@10} & \textbf{NDCG@10} \\ 
% \midrule
\hline
\textbf{(0) Default}                                    & \textbf{0.3576}      & \textbf{0.2931}    & \textbf{0.1863}    & \textbf{0.1073}  \\ 
(1) w/o \textit{TE}-$\phi(\cdot)$                                & 0.3485               & 0.2819             & 0.1683             & 0.0933           \\
(2) w/o \textit{GE}-$d(\cdot,\cdot)$                                    & 0.2505               & 0.1781             & 0.0953             & 0.0501           \\
% \bottomrule
\hline
\end{tabular}
}
\vspace{-0.1in}
\end{table}

==> 04other/050related.tex <==




% \subsection{POI Recommendation}

\textbf{Next POI Recommendation.} 
Most of the earlier works \cite{liu2016predicting,feng2018deepmove,sun2020go,lian2020geography,ma2018point,luo2021stan} adopt sequential methods, such as RNN \cite{medsker2001recurrent} and self-attention \cite{vaswani2017attention}, to capture spatial and temporal contexts.
ST-RNN \cite{liu2016predicting} uses temporal and spatial intervals between adjacent items in a RNN to improve model performance.
This usage of intervals has also been applied in other sequential methods \cite{lian2020geography,ma2018point,luo2021stan}.
% For instance, SAE-NAD \cite{ma2018point} adopts a self-attentive encoder and a neighbor-aware decoder to incorporate the geographical information.
Besides, some recent works \cite{feng2018deepmove,sun2020go,cui2021st} aim to capture the multi-level periodicity of user preferences from long-term behaviors through the attention mechanism.
% Recently, \cite{christoforidis2018recommendation,han2020stgcn,kim2021dynaposgnn,yang2022getnext} adopt graph-based methods to exploit the extensive collaborative signals for user-POI, POI-POI, or POI-region relations.
For instance, ST-PIL \cite{cui2021st} designs both the long-term and short-term modules to learn the periodic interest.
However, these methods, which learn long and short-term preferences, still have a limited ability to explicitly encode the region-aware periodic.
In summary, the region-aware periodic problem for local-life service recommendation is not well-addressed in these methods. 

% \subsection{Temporal Graph Neural Networks}

\noindent\textbf{Periodic-related Recommenders.} 
Temporal evolution is an important factor for user preference modeling.
% Earlier works \cite{wu2019sessionbased,kang2018selfattentive,sun2019bert4rec} attempt to capture dynamic user preference by sequential methods from historical long sequences without explicitly encoding the interaction periodic.
Some recent works \cite{wang2019modeling,fan2021continuoustime,rossi2020temporal,tian2022temporal} attempt different utilization of time intervals with time-decaying functions to capture the periodicity of user preferences.
For instance, TGSRec \cite{fan2021continuoustime} and TGN \cite{rossi2020temporal} utilize generic time encoding functions to explicitly encode the periodicity.
SLRC \cite{wang2019modeling} proposes a Hawkes process into collaborative filtering for repeat consumption.
However, these methods fail to utilize the spatial-temporal contexts to model the region-aware periodic for local-life service recommendation.

% Temporal graph neural networks \cite{kumar2019predicting,trivedi2019dyrep,xu2020inductive,rossi2020temporal} have been a huge success in many tasks \cite{skarding2021foundations}. 
% For instance, TGN \cite{rossi2020temporal} first proposes a unified framework for temporal link prediction. 
% Recently, some works \cite{fan2021continuoustime,zhang2022dynamic,chi2022long} have applied temporal graph neural networks to capture temporal evolution and periodic for the continuous-time recommendation. 
% However, to the best of our knowledge, there are few works that simultaneously capture the interaction periodic and region periodic for local-life service recommendation.

==> 04other/060conclusion.tex <==




In this paper, we first study how to solve the region-aware periodic problem for local-life service recommendation, which has rarely been studied by previous works.
To address the issue, we propose a novel \modelname. 
To capture the spatial-temporal contexts for periodic modeling, we design the periodic encoding with temporal encoding and geographical encoding. 
To further capture the region-aware periodic, we propose the geographical temporal graph transformer with periodic encoding.
Extensive experiments on both real-world public and industrial datasets demonstrate the effectiveness of our proposed \modelname. 
For future work, we plan to deploy online A/B tests to further evaluate the performance.
% In future work, we will push forward the implementation of \modelname in Meituan's local-life services.
